A Computer Vision Approach for Autonomous Cars to Drive Safe at Construction Zone

To build a smarter and safer city, a secure, efficient, and sustainable transportation system is a key requirement. The autonomous driving system (ADS) plays an important role in the development of smart transportation and is considered one of the major challenges facing the automotive sector in recent decades. A car equipped with an autonomous driving system (ADS) comes with various cutting-edge functionalities such as adaptive cruise control, collision alerts, automated parking, and more. A primary area of research within ADAS involves identifying road obstacles in construction zones regardless of the driving environment. This paper presents an innovative and highly accurate road obstacle detection model utilizing computer vision technology that can be activated in construction zones and functions under diverse drift conditions, ultimately contributing to build a safer road transportation system. The model developed with the YOLO framework achieved a mean average precision exceeding 94\% and demonstrated an inference time of 1.6 milliseconds on the validation dataset, underscoring the robustness of the methodology applied to mitigate hazards and risks for autonomous vehicles.

==> draft.tex <==
Data drift in image data can significantly impact autonomous driving systems, particularly object detection models.  It occurs when the distribution of the input images changes over time, different from the original training data. This can happen due to various factors such as environmental changes, infrastructure updates, vehicle modifications, etc.  It can cause decreased accuracy, reduce reliability, and increase risk of safety. To address data drift in autonomous driving systems, several techniques such as continuous monitoring, regular model updates, adaptive learning techniques, robust data collection, and simulation and enhancement. By addressing data drift, developers of autonomous driving systems can ensure that their object detection models remain accurate, reliable, and safe in the face of changing real-world conditions. This is crucial to maintaining the performance and safety of self-driving vehicles as they navigate diverse and dynamic environments.
\begin{figure}[!h]
    \centering
    \subfloat[Barrier]{\label{fig:std1}
        \includegraphics[width=0.16\textwidth]{map01D_11.png}}
    \hspace{1cm} % Adjust the horizontal space between images if needed
    \subfloat[Beacon]{\label{fig:drift2}
        \includegraphics[width=0.16\textwidth]{map01D_64.png}}
    \hspace{1cm}
    \subfloat[Cone]{\label{fig:drift3}
        \includegraphics[width=0.16\textwidth]{map01D_83.png}}
    \caption{Different Obstacles}
    \label{fig:drift}
\end{figure}

As self-driving cars accumulate more data from real-world driving scenarios, their algorithms become more refined and able to handle a wide range of situations.  Furthermore, ML in automotive applications can learn continuously and improve performance from experience. This iterative learning process is essential for the development of robust autonomous systems that can operate safely in various environments. In addition, machine learning is not limited to fully autonomous vehicles. It also plays an important role in improving driver assistance functions in conventional cars, such as parking warnings, adaptive cruise control, and collision detection systems. These features offered by Ml significantly improve road safety by strengthening the abilities of human drivers and preventing accidents caused by human mistakes. As the automotive industry continues to evolve, machine learning will undoubtedly play an increasingly important role in the future of transportation, from improving vehicle performance and efficiency to enabling new levels of autonomy and safety on the roads.
